Morpheus: Automated Safety Verification of Data-dependent Parser Combinator Programs

Parser combinators are a well-known mechanism used for the compositional construction of parsers, and have shown to be particularly useful in writing parsers for rich grammars with data-dependencies and global state. Verifying applications written using them, however, has proven to be challenging in large part because of the inherently effectful nature of the parsers being composed and the difficulty in reasoning about the arbitrarily rich data-dependent semantic actions that can be associated with parsing actions. In this paper, we address these challenges by defining a parser combinator framework called Morpheus equipped with abstractions for defining composable effects tailored for parsing and semantic actions and a rich specification language used to define safety properties over the constituent parsers comprising a program. Even though its abstractions yield many of the same expressivity benefits as other parser combinator systems, Morpheus is carefully engineered to yield a substantially more tractable automated verification pathway. We demonstrate its utility in verifying a number of realistic, challenging parsing applications, including several cases that involve non-trivial data-dependent relations.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> evaluation-rules-basic.tex <==
\subsection{SafeParse Primitive Parser Expressions Semantics}

\newcommand{\context}{E}
\newcommand{\ALT}{\mid}

\begin{array}{lcc}
\context & ::= & \bullet \ALT \context(\eip) \ALT \context\, [\mathsf{t}] %%
     \ALT v(\context) \ALT \mathsf{ref}_p \context \ALT \mathsf{deref}_p \context %%
     \ALT E\, :=\, \eip \ALT \ell_p \, := E\\
&    \ALT \mathbf{match}\, E\, \mathbf{with}\, \mathsf{D_i}\, %%
             \overline{\alpha}\, \overline{\xp_{j}} \rightarrow \eip %%
             \ALT \mathbf{if}\ E\ \mathbf{then}\ \eip\, \mathbf{else}\, \eip\\
&    \ALT \mathbf{return}\, E \ALT \mathbf{let}\, x\, = E in \eip\\
&    \ALT E\, (>>=)\, \eip \ALT\ E\ (<\mid>)\, \eip 
\end{array}


\begin{figure}[h]
\begin{flushleft}
\fbox{\small
        $(\mathcal{H}; \mathsf{\eip}) \Downarrow (\mathcal{H'}; \mathsf{\vp}) $ 
           
} 
\bigskip
\end{flushleft}
% \begin{minipage}{0.4\textwidth}
% \small \begin{center}
% \inference[{\sf E-dref}]{ (\mathcal{H}; {\sf e}) \rightarrow (\mathcal{H'}; {\sf e'})}
% 				  {(\mathcal{H}; {\sf ! e}) \rightarrow 
% (\mathcal{H'}; {\sf ! e'})) } 
% 
% \end{center}

%\end{minipage}
\begin{minipage}{0.5\textwidth}
\small \begin{center}
\inference[{\sf E-dref-loc}]{ \mathcal{H}(l) = {\sf \vp}}
				  {(\mathcal{H}; {\sf ! l}) \Rightarrow 
(\mathcal{H}; {\sf v}) } 
\end{center}
\end{minipage}
\bigskip
\begin{minipage}{0.4\textwidth}
\small \begin{center}
\inference[{\sf E-assign}]{ }{(\mathcal{H}; {\sf l := v}) \Rightarrow 
(\mathcal{H}[{\sf l \mapsto v}]; {\sf unit})) } 
\end{center}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\small \begin{center}
\inference[{\sf E-ref}]{ l \in {\sf dom} (\mathcal{H}) }
				  {(\mathcal{H}; {\sf ref \ v}) \Rightarrow 
((\mathcal{H}, {\sf l \mapsto v}); {\sf l}) } 
\end{center}
\end{minipage}
\bigskip
\begin{minipage}{0.4\textwidth}
\small \begin{center}
\inference[{\sf E-if-true}]{ (\mathcal{H}; e_1) \Rightarrow  (\mathcal{H'}; {\sf v})}
	{(\mathcal{H}; {\sf if \ true \ then e_1 \ else \ e_2}) \Rightarrow 
(\mathcal{H'}; {\sf v})} 
\end{center}

\end{minipage}

\begin{minipage}{0.5\textwidth}
\small \begin{center}
\inference[{\sf E-if-false}]{ (\mathcal{H}; e_2) \Rightarrow  (\mathcal{H'}; {\sf v})}
	{(\mathcal{H}; {\sf if \ true \ then e_1 \ else \ e_2}) \Rightarrow 
(\mathcal{H'}; {\sf v})} 
\end{center}
\end{minipage}

\bigskip
\begin{minipage}{0.4\textwidth}
\small \begin{center}
\inference[{\sf E-match}]{ (\mathcal{H}, [\overline{\mathsf{v}_{j}}/ \overline{\mathsf{x}_{j}}]\eip) \Rightarrow
(\mathcal{H'}; {\sf v})}
{(\mathcal{H}; {\bf match} \ \mathsf{D_i}) 
\overline{\mathsf{v}_{j}} \ {\bf with} \ \mathsf{D_i} 
\overline{\mathsf{x}_{j}} \rightarrow \eip) \Rightarrow 
(\mathcal{H}, {\sf v})} 
\end{center}
\end{minipage}

\begin{minipage}{0.5\textwidth}
\small \begin{center}
\inference[{\sf E-ret}]{(\mathcal{H}; e) \Rightarrow 
(\mathcal{H},  {\sf v}) }{(\mathcal{H}; {\bf return} \ e) \Rightarrow 
(\mathcal{H}, {\sf v})} 
\end{center}
\end{minipage}
\bigskip

% Move too appendix
%\begin{minipage}{0.4\textwidth}
% \small \begin{center}
% \inference[{\sf E-typeapp}]{  }{} 
% \end{center}
% \end{minipage}
% 
% \begin{minipage}{0.5\textwidth}
% \small \begin{center}
% \inference[{\sf E-funapp}]{  }{} 
% \end{center}
% \end{minipage}
% 
\caption{Evaluation rules for $\lambda_{sp}$ base-expressions}
\label{fig:semantics-base}
\end{figure}


==> intro-example.tex <==
\section{Motivating Example}
\label{sec:ex}



To highlight the challenges in verification, we consider a motivating example based on a
particular class of stateful parsers that are {\it
  indentation-sensitive}, and which are widely used in many functional
language implementations. These parsers are characterized by having
indentation or layout as an essential part of their grammar. Because
indentation sensitivity cannot be specified using a context-free
grammar, their specification is often specified via an orthogonal set
of rules, for example, Haskell's offside
rule.\footnote{https://www.haskell.org/onlinereport/haskell2010/haskellch10.html}
The Haskell parser implements these rules in a complex routine found
in the lexing phase of the compiler. Other indentation-sensitive
languages like Idris~\cite{idris} use parsers written using a parser
combinator libraries like \S{Parsec} or its
variants~\cite{parsec,megaparsec}.

\begin{figure}
\begin{subfigure}[t]{0.48\textwidth}
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,breaklines=true,showspaces=false,
  showstringspaces=false, tabsize=2, breaklines=true,
  xleftmargin=5.0ex]
 DoBlock ::= 'do' OpenBlock Do* CloseBlock;
 Do ::=
    'let' Name  TypeSig'      '=' Expr
   | 'let' Expr'                '=' Expr
   |  Name  '<-' Expr
   |  Expr' '<-' Expr
   |  Ext Expr
   |  Expr  
   ;
\end{lstlisting}
\caption{An Idris grammar rule for a {\sf do} block}
\label{fig:idris-grammar}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}  
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,breaklines=true,showspaces=false,
  showstringspaces=false, tabsize=2, breaklines=true,
  xleftmargin=5.0ex]
  expr =  do 
            t <- term 
  	        symbol "+" 
	          e <- expr 
	          pure t + e
         symbol '*'      
\end{lstlisting}
\caption{An input to the parser.}
\label{fig:idris-grammar-example}
\end{subfigure}
\caption{An Idris grammar rule for a {\sf do} block and an example input.}
\end{figure}

To illustrate how parser combinators can be used to specify
indentation sensitivity, consider the Idris grammar fragment shown in
Figure~\ref{fig:idris-grammar}.  The grammar defines the rule to parse
a \S{do}-block. Such a block begins with the \S{do} keyword, and is
followed by zero or more \S{do} statements that can be \S{let}
expressions, a binding operation ($\leftarrow$) over names and
expressions, an external expression, etc. The Idris documentation
specifies the indentation rule in English governing where these
statements must appear, saying that the ``\emph{indentation of each
  \S{do} statement in a \S{do}-block {\sf Do*} must be greater than
  the current indentation from which the rule is
  invoked}~\cite{idrisgrammar}.'' Thus, in the Idris code fragment
shown in Figure~\ref{fig:idris-grammar-example}, the indentation
sensitivity constraints require that the last statement is not a part
of the do-block, while the inner three statements are. A correct Idris
parser must ensure that such indentation rules are preserved.

Figure~\ref{fig:idris-original-do} presents a fragment of the parser
implementation in Haskell for the above grammar, taken from the Idris
language implementation source, and simplified for ease of
explanation. The implementation uses Haskell's \S{Parsec} library, and
since the grammar is not context-free, it implements indentation rules
using a state abstraction (called {\sf IState}) that stores the
current indentation. The parser then manually performs reads and
updates to this state and performs indentation checks at appropriate
points in the code (e.g. line~\ref{line:lo1}).

\begin{figure}
\begin{subfigure}[t]{0.5\textwidth}
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,numbers=left,language=Haskell,showstringspaces=false]
data IState = IState {
    ist :: Int
    @\dots@
} deriving (Show)

data PTerm =  PDoBlock [PDo]                               
data PDo t =  DoExp t | DoExt t | DoLet  t t | @\ldots@            
type IdrisParser a = Parser IState a @\label{line:idrisp}@

getIst :: IdrisParser IState
getIst = get 
putIst :: (i : Int) -> IdrisParser ()
pustIst i = put {ist = i}

doBlock :: IdrisParser PTerm
doBlock = do  
            reserved "do"
            ds <- indentedDoBlock
            return (PDoBlock ds)
indentedDo ::  IdrisParser (PDo PTerm)
indentedDo = do 
               allowed <- ist getIst @\label{line:getind}@
               i <- indent
               if (i <= allowed) @\label{line:lo1}@
                  then fail ("end of block")
               else   
                  do_ @\label{line:originaldo}@   
\end{lstlisting}
\end{subfigure}
\begin{subfigure}[t]{0.48\textwidth}
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,numbers=left,breaklines=true,firstnumber=28,language=Haskell,showstringspaces=false]
do_ :: IdrisParser (PDo PTerm)
do_  =  do 
          reserved "let"
          i <- name
          reservedOp "="
          e <- expr 
          return (DoLet i e)
    <|> do 
          i <- extension
          e <- expr 
          return (DoExt  i e)
    <|> do e <- expr 
           return (DoExp  e)
indentedDoBlock :: IdrisParser [PDo PTerm]
indentedDoBlock  = @\label{line:indentdostart}@
    do 
        allowed <- ist getIst @\label{line:indentdobegin}@  
        lvl' <- indent 
        if (lvl' > allowed) then @\label{line:indentGreater2}@
            do 
                putIst lvl' @\label{line:setind}@ 
                res <- many (indentedDo) @\label{line:many}@ 
                putIst allowed @\label{line:reset}@
                return res 
        else 
            fail "Indentation error"
indent :: IdrisParser Int
indent = P.unPos . P.sourceColumn @\$@ 
                    P.getSourcePos
\end{lstlisting}
\end{subfigure}
\caption{A fragment of a \S{Parsec} implementation for Idris \S{do}-blocks with indentation checks.}
\label{fig:idris-original-do}
\end{figure}
The IdrisParser (line~\ref{line:idrisp}) is defined in terms of
\S{Parsec}'s parser monad over an Idris state (here, {\sf IState}), which
along with other fields has an integer field (\S{ist}) storing the
current indentation value.  A typical indentation check (e.g. see
lines~\ref{line:getind} - ~\ref{line:lo1}) fetches the current value
of \S{ist} using \S{getIst}, fetches the indentation of the next
lexeme using the \S{Parsec} library function \S{indent}, and compares
these values.

The structure of the implementation follows the grammar
(Figure~\ref{fig:idris-grammar}): the {\sf doBlock} parser parses a
reserved keyword ``\S{do}'' followed by a block of \S{do\_} statement
lists.  The indentation is enforced using the parser
\S{indentedDoBlock} (defined at line~\ref{line:indentdostart}) that
gets the current indentation value (\S{allowed}) and the indentation for
the next lexeme using \S{indent}, checks that the indentation is
greater than the current indentation (line~\ref{line:indentGreater2})
and updates the current indentation so that each \S{do} statement is
indented with respect to this new value. 

\begin{wrapfigure}{r}{.5\textwidth}
  \vspace*{-.2in}
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,breaklines=true,language=Haskell, numbers=left, showspaces=false,
  showstringspaces=false, tabsize=2, breaklines=true,
  xleftmargin=5.0ex]
  expr = do 
            t <- term 
	          do 
              symbol "+" 
	            e <- expr 
	            pure  t + e
	       "mplus" pure t
\end{lstlisting}
\caption{An input expression that is incorrectly parsed by the implementation shown in Figure~\ref{fig:idris-original-do}.}
\label{fig:inputexample}
\vspace*{-.20in}
\end{wrapfigure}

It then calls a parser
combinator {\sf many} (line~\ref{line:many}), which is the \S{Parsec}
combinator for the Kleene-star operation, over the result of
\S{indentedDo}, i.e., $\mathsf{indentedDo}^{*}$.  The {\sf
  indentedDo} parser again performs a manual indentation check,
comparing the indentation value for the next lexeme against the
block-start indentation (set earlier by {\sf indentedDoBlock} at line
~\ref{line:setind}) and, if successful, runs the actual \S{do\_}
parser (line~\ref{line:originaldo}).  Finally, {\sf indentedDoBlock} resets
the indentation value to the value before the block
(line~\ref{line:reset}).

Unfortunately, it is non-trivial to reason that these manual checks
suffice to enforce the indentation sensitivity property we desire.
Since they are sprinkled throughout the implementation, it is easy to
imagine missing or misplacing a check, causing the parser to
misbehave. More significantly, the implementations like these may make incorrect
assumptions about the effectful actions performed by the library that
are reflected in the API signatures. In fact, the logic in the above
code has a subtle bug~\cite{indentation1} that manifests in the
input example shown in Figure~\ref{fig:inputexample}.

%\TODO{Indentation in this figure, use something other than listing}
Note that the indentation of the token ``mplus'' is such that it is
not a part of either \S{do} block; the implementation, however, parses
the last statement as a part of the inner do-block, thereby violating the
indentation rule, leading to the program being incorrectly parsed.

The problem lies in a mismatch between the contract provided by the
library's \S{indent} function and the assumptions made about its
behavior at the check at line~\ref{line:lo1} in the {\sf indentedDo}
parser. Since checking indentation levels for each character is
costly, \S{indent} is implemented in a way that causes certain lexemes
to be ignored during the process of computing the next indentation
level. In this example, {\sf indent} does not check the indentation of
lexeme ``mplus'', returning the indentation of the token  \S{pure} instead.  Thus, the indentation of the last statement is considered
to start at \S{pure}, which incorrectly satisfies the checks at
line~\ref{line:lo1} or line~\ref{line:indentGreater2}, and thus causes
this statement to be accepted as part of \S{indentedDoBlock}.

Unfortunately, unearthing and preventing such bugs statically is
challenging for two reasons. First, the specification of the required
safety property, i.e. the {\it indentation of the next lexeme parsed
  must be in the allowed range of indentation values}, relates two
values in the mutable state, {\sf ist} and the {\sf inp} and thus
requires stateful specifications which are beyond the capabilities of Haskell's
core type system, to express. Second, the parser combinator library
exposes effectful computation operating over internal states,
exceptions, and non-deterministic choices (\S\small{<|>}), as seen, for
example, in the definition of \S{do\_}; reasoning about the scope and
nature of these effects is additionally complicated by the
expressivity of the host language that weaves calls to these
combinators through arbitrarily complex control- and dataflow.

To address the first challenge, we express effectful specifications in
\name\ as refinement types~\cite{refinementTypeTutorial}, equipped
with a decidable type-checking procedure. Our type system allows the
specification of both parser-local stateful actions as well as more
global combinator-based effects, allowing small-footprint
specifications and modular verification. To address the second
challenge, \name\ axiomatizes the definition of a set of core
primitive parser combinators and constrains the kinds of state changes
they are allowed to perform by design. Further \name restrict their interaction
with the host language via a simplified memory abstraction that is
nonetheless sufficient to express and verify a wide range of
interesting parser combinator-based programs. Our design choices are
chosen to enable the generation of verification conditions that can be
discharged using off-the-shelf SMT solvers, thus enabling automation.
The combinators provided by our DSL thus serve as a kernel for writing
more complex derived combinators whose types can be automatically
synthesized by \name.





==> overview.tex <==
\section{\name\ Overview}
\label{sec:overview}
% When, Why  How, What , Where

In this section, we provide an overview of Morpheus by adapting our
introductory example to its setting.

\subsection{Surface Language}
An important design decision we make is to provide a surface syntax
and API very similar to a conventional monadic parser combinator
libraries like \S{Parsec}~\cite{parsec} in Haskell or
\S{mParser}~\cite{mparser} in OCaml; the core API that \name\ provides
has the signature shown in Figure~\ref{fig:api}. The library defines
a number of primitive combinators: \S{eps} defines a parser for the
empty language, \S{bot} always fails, and \S{char \ c} defines a
parser for character \S{c}. Beyond these, the library also provides a
bind (\S{>>=}) combinator for monadically composing parsers, a choice
\begin{wrapfigure}{r}{.40\textwidth}
  \begin{center}
  \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,breaklines=true,language=ML, showspaces=false]
    type 'a t
    val eps : unit t
    val bot : 'a t
    val char : char -> char t 
    val (>>=) : 'a t -> (a -> 'b t) -> 'b t 
    val <|> : 'a t -> 'a t -> 'a t 
    val fix : ('b t -> 'b t) -> 'b t
  \end{lstlisting}
  \end{center}
  \caption{Signatures of primitive parser combinators supported by \name.}
  \label{fig:api}
  \vspace*{-.2in}
  \end{wrapfigure}
({<|>}) combinator to non-deterministically choose among two parsers,
and a \S{fix} combinator to implement recursive parsers. As we
demonstrate, these combinators are sufficient to derive a number of
other useful parsing actions such as \S{many}, \S{count}, etc. found
in these popular combinator libraries. From the parser writer's
perspective, \name\ programs can be expressed using these combinators
along with a basic collection of other non-parser expression forms
similar to those found in an ML core language, e.g., first-class
functions, \S{let} expressions, references, etc.
For instance, we can define an always successful parser, {\sf return x}, as follows:
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
  let return x = @$\lambda \_$@. x
\end{lstlisting}
Similarly, a parser for {\sf option p}, which either parses an empty string or anything that 
{\sf p} parses can be written:
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
  let option p = (eps >>= @$\lambda$@ $\_$. return None) <|> (p >>= @$\lambda$@ x. return Some x) \end{lstlisting}
We can also define more intricate parsers like {\it Kleene-star} and {\it Kleene-plus}:
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
  let star p = fix ($\lambda$ p_star. eps  <|> p >>= @$\lambda$@ x. p_star >>= @$\lambda$@ xs . return (x :: xs) ) 
  let plus p = fix ($\lambda$ p_star. p  <|> p >>= @$\lambda$@ x. p_star >>= @$\lambda$@ xs . return (x :: xs) ) 
\end{lstlisting}
Figure~\ref{fig:idris-do} shows a \name implementation for a portion
of the Idris {\sf doBlock} parser from
Figure~\ref{fig:idris-original-do} showing the implementation of three
parsers for brevity, {\sf doBlock}, {\sf indentedDo}, and {\sf
  indent}. The structure is similar to the original Haskell
implementation, even though the program uses ML-style operators for assignment
and dereferencing. For ease of presentation, we have written the
program using {\it do-notation} (\M{do}) as syntactic sugar for
\name's monadic bind combinator.
% @\texttt{\textcolor{gray}{
%  \begin{tabbing}                        
%  indentedDo : \label{line:indentedDospec} \\
%  $\mathsf{PE^{state}}$\,\= \{sel\= (h, ist) = I\}\\ 
%  \>\>              v : offsideTree I  \\
%  \{indentT (v) = pos (sel (h, inp)\}
%  \end{tabbing}}}@

\begin{figure}
  \begin{subfigure}[t]{0.45\textwidth}
  \begin{lstlisting}[escapechar=\@,basicstyle=\footnotesize\sf,numbers=left,language=ML,showspaces=false,showstringspaces=false,tabsize=1]
type @$\alpha$@ pdo  =  DoExp of @$\alpha$@ | DoExt of @$\alpha$@ | @\ldots@    
type pterm =  PDoBlock of ((pterm pdo) list)                        
let ist = ref 0
@$\ldots$@
@\texttt{\textcolor{blue}{
\begin{tabbing}
doBlock :\\ \label{line:doBlockSpec}
$\mathsf{PE^{state}}$\=\\
\>\{$\forall$ h, I. sel\= (h, ist) = I\} \\
\>\quad            $\nu$ : offsideTree I  \\
\>\{$\forall$ h, $\nu$, h', I, I'.\=\\
\>\,\,(sel (h, ist) = I $\wedge$ \\
\>\,\,\, sel (h', ist) = I') => I' = I\}
 \end{tabbing}}}@
let doBlock @\label{line:doblock}@ = 
    @\M{do}@ 
       dot <- reserved "do" @\label{line:do}@
       ds  <- indentedDoBlock @\label{line:ds}@
       return Tree {term = PDoBlock ds; @\label{line:l1}@
                   indentT = indentT (dot);
                   children = (dot :: ds) @\label{line:lcons}@}
@\texttt{\textcolor{gray}{
   \begin{tabbing}
     do\_ : $\mathsf{PE^{state}}$\=
\{sel\= (h, inp) = I\} \label{line:dospec}\\  
\>\quad              $\nu$ : tree    \\
\{indentT($\nu$) = pos (sel (h, inp)) $\wedge$ \\
\>\,\, children ($\nu$) = nil\}
   \end{tabbing}}}@                     
let do_ = @$\ldots$@
\end{lstlisting}
  \end{subfigure}
  \begin{subfigure}[t]{0.48\textwidth}
  \begin{lstlisting}[escapechar=\@,basicstyle=\footnotesize\sf,numbers=left,breaklines=true,firstnumber=15,language=ML,showstringspaces=false]
@\texttt{\textcolor{gray}{
  \begin{tabbing}                        
   $\mathsf{PE^{state}}$\,\= \{sel\= (h, ist) = I \}\\ \label{line:inferredindentDo}
  \>\>      $\nu$ : tree option  \\
  \{
  $\forall$ i : int.  
   $\nu$ = \S{Inl} x $\Rightarrow$ i > I $\wedge$ \\
    indentT (x) = pos (sel (h, inp) $\wedge$ \\
    children (x) = nil \\
  $\wedge$ $\nu$ = \S{Inr} Err $\Rightarrow$  i <= I $\wedge$ h' = h\}
  \end{tabbing}}}@
let indentedDo = @\label{line:idostart}@ 
    @\M{do}@ 
       allowed <- !ist
       i <- indent @\label{line:indentcall}@ 
       if (i <= allowed ) @\label{line:l3}@ then 
           fail ("end of block")
       else    
            do_ @\label{line:l4}@ 
@\texttt{\textcolor{gray}{  
\begin{tabbing}
sourceColumn : (char * int) list -> int \label{line:sc}
\end{tabbing}
}}@
let sourceColumn = @$\ldots$@
@\texttt{\textcolor{gray}{  
\begin{tabbing}
indent : \label{line:indentspec}
$\mathsf{PE^{state}}$ \{true\}\,
        $\nu$ : int\, \{ h' = h \}
\end{tabbing}
}}@ 
let indent = 
    @\M{do}@
      s <- !inp
      let column = sourceColumn s 
      return column  

 \end{lstlisting}
  \end{subfigure}
  \caption{\name\ implementation and specifications for a portion of
    an Idris \S{Do}-block with indentation checks, \M{do} is a
    syntactic sugar for \name's monadic bind.  Specifications given in
    \textcolor{blue}{Blue} are provided by the parser writer;
    \textcolor{gray}{Gray} specifications are inferred by \name.}
  \label{fig:idris-do}
  \end{figure}


\subsection{Specifying Data-dependent Parser Properties}
To specify an \emph{indentation-sensitivity} safety property, we first
define an inductive type for a parse-tree (\S{tree}) and refine this
type using a dependent function type, ({\sf offsideTree i}), that
specifies an indentation value for each parsed result.
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
  type tree = Tree {term : pterm; indentT : int; children : tree list}
  type offsideTree i = Tree {term : pterm; @\label{line:tree}@ indentT : { v : int | v > i }; children : (offsideTree i) list}
 \end{lstlisting}
This type defines a tree with three fields:
\begin{itemize}
\item A \S{term} of type {\sf pterm}. 
%where \S{pterm} is the
%\name\ equivalent of the original parser implementation return type
%\S{PTerm} shown in Figure~\ref{fig:idris-original-do}.
\item The indentation (\S{indentT}) of a returned parse tree defined
  in terms of the tree's first grammar symbol, with a refinement that
  requires its indentation to be greater than \S{i}.
\item A list of sub-parse trees (\S{children}) for each of the
  terminals and non-terminals in the current grammar rule's right-hand
  side, each of which must also satisfy this refinement.
\end{itemize}
\name\ additionally introduces {\it qualifiers} for each of the
datatype's constructors and fields with the same name that can be used
in type refinements.
%% E.g. for the tree type, \name
%% generates three qualifiers {\it viz.} tree, indentT and children.
%% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%%  qualifier term : tree -> pterm
%%  qualifier indentT : tree -> int 
%%  qualifier children : tree -> tree list 
%% \end{lstlisting}
The type {\sf offsideTree i} is sufficient to specify pure functions
that return an indented tree, e.g.,
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
  goodTree : (i : int) -> offsideTree i
\end{lstlisting}
However, such types are not sufficiently expressive to specify
stateful properties of the kind exploited in our example program. For
example, using this type, we cannot specify the required safety
property for {\sf doBlock} that requires ``{\it the indentation of the
  parse tree returned by {\sf doBlock} must be greater than the current
  value of \S{ist}}'' because \S{ist} is an effectful heap variable.

\paragraph{Specifying effectful safety properties}
To specify effectful properties, our specification language also
provides a type for effectful computations. We use a specification
monad of the form $\mathsf{PE^{\el}}$ \{ $\phi$ \} $\nu$ : $\tau$ \{
$\phi'$ \} that is parameterized by the \emph{effect} of the
computation $\el$ (e.g., \S{state}, \S{exc}, etc.), and Hoare-style
pre- and post-conditions~\cite{htt,fstar,vcc}. Here, $\phi$ and
$\phi'$ are first-order logical propositions over qualifiers applied
to program variables and variables in the type context.  The
precondition $\phi$ is defined over an abstract input heap {\sf h}
while the postcondition $\phi'$ is defined over input heap {\sf h},
output heap {\sf h'}, and the special result variable $\nu$ that denotes
the result of the computation.  Using such types, we can specify a
safety property for a {\sf doBlock} parser as shown on
line~\ref{line:doBlockSpec} in Figure~\ref{fig:idris-do}.

The type should be understood as follows: The precondition binds the
value of the mutable state variable {\sf ist}, a reference to the
current indentation level, to {\sf I} via the use of the built-in
qualifier \S{sel} that defines a select operation on the
heap~\cite{mccarthy}.  The return type (\S{offsideTree\ I}) obligates
the computation to return a parse tree whose indentation must be
greater than {\sf I}. The postcondition constrains that the final
value of the indentation is to be reset to its value prior to the
parse (a \emph{reset} property).  The types for other parsers in
the figure can be specified as shown at lines ~\ref{line:dospec},
~\ref{line:inferredindentDo}, ~\ref{line:indentspec}, etc.; these types are automatically inferred
by \name's type inference algorithm. For example, the type for the
{\sf do\_} parser (line ~\ref{line:dospec}) returns a base type {\sf
  tree} and uses a integer-valued qualifier {\sf pos} over an indexed
list giving the head position of the list. Intuitively the type says
that the indentation of the returned tree is equal to the index of the
first character in the input, and there are no children in the tree.
Similarly, the postcondition for parser \textsf{indent} asserts the
parser makes no modification to the program heap, a claim consistent
with its implementation that only uses pure function
\textsf{sourceColumn} to return the current indentation position.

%% \subsection{Type Checking}
%% %\AM{What : Talk about doBlock parser and its verification
%%  % How : Example} Given a \name implementation and specification,
%% Given a \name implementation and specification, \name's type-system
%% allows us to verify if the implementation for the parser satisfies a
%% data-dependent safety property.  





%% Consider the subparser {\sf
%%   indentedDo} shown in Figure~\ref{fig:idris-do}.  Given the
%% top-level goal specification for {\sf indentedDo} is given by the
%% programmer (shown in \textcolor{blue}{blue}) while those
%% specifications in \textcolor{gray}{gray} are inferred by \name.  For
%% perspicuity, we have elided the implementations of some functions like
%% {\sf do\_} and {\sf sourceColumn} while only showing their
%% specifications.  The {\sf sourceColumn} (line~\ref{line:sc}) is a pure
%% function which given the the list of input tagged with integer indices
%% returns an index value from the list. Thus, the type inferred for {\sf
%%   indent} (line~\ref{line:indentspec}) has the {\sf pure} effect and
%% consequently, the post condition captures that the heap is unchanged
%% (i.e. {\sf \{ h' = h\}}).

% To verify that the \S{doBlock} implementation (line~\ref{line:doblock}) correctly matches its specification, we need
% to prove that the tree returned at line ~\ref{line:l1} is well-typed
% (i.e. it has type {\sf offsideTree I}) for the value \S{I} given in
% its precondition and that the resulting tree satisfies the
% \emph{indentation} properties described above (we elide the {\it reset} property discussion here for elucidation). 
% To do
% this, we first need to show that the result of parsing the terminal
% {\sf ``do''}, i.e. the value bound to {\sf dot} also satisfies these
% conditions, and second, that the result of parsing a block of \S{do}
% statements, i.e. {\sf ds}, has the type {\sf (offsideTree I) list}.
% %and satisfies the \emph{reset} property as well.
% Let us focus our attention to see how \name verifies the second goal,
% i.e. {\sf children} (line~\ref{line:lcons}) has a type ({\sf
%   (offsideTree I) list}). 
  

% First, the type for the polymorphic list
% (used at line~\ref{line:lcons}) will be instantiated with the current
% type of list elements (i.e. (offsideTree i)) as follows. Note that
% \name syntax for refined typed definition is similar to OCaml type
% definition.
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% type (offsideTree i) list =  nil | cons of offSideTree i * (offsideTree i) list
% \end{lstlisting}
% Thus to prove that {\sf ds} (line~\ref{line:ds}) is a list of {\sf
%   offsideTree I} (i.e., trees whose \S{indentT} value is greater
% than \S{I}), we need to prove that the result of the 
% {\sf indentedDoBlock} parser has the type {\sf (offSideTree I) list}.
% Note that although \name infers a type for the {\sf indentedDoBlock}, for elucidation purposes, let us assume that we give a required type for the {\sf indentedDoBlock} based on the above argument, thus showing the line~\ref{line:indentedDoBlockspec} in \textcolor{blue}{blue}.


  
% \paragraph{Handling Stateful expressions and Higher-Order Combinators}
% %\AM{What : \name Combinators, HOW : Example}
% Let us focus our attention to see how \name verifies the second goal,
% i.e. {\sf children} (line~\ref{line:lcons}) has a type ({\sf
%   (offsideTree I) list}).  First, the type for the polymorphic list
% (used at line~\ref{line:lcons}) will be instantiated with the current
% type of list elements (i.e. (offsideTree i)) as follows. Note that
% \name syntax for refined typed definition is similar to OCaml type
% definition.
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% type (offsideTree i) list =  nil | cons of offSideTree i * (offsideTree i) list

% \end{lstlisting}
% Thus to prove that {\sf ds} (line~\ref{line:ds}) is a list of {\sf
%   offsideTree I} (i.e., trees whose \S{indentT} value is greater
% than \S{I}), we need to prove that the result of the 
% {\sf indentedDoBlock} parser has the type {\sf (offSideTree I) list}. 
% There are two main challenges in proving the above goal:
% \begin{itemize}
% \item Effectful semantics of expressions, 
% {\it viz.} the {\sf deref} expressions like {\sf allowed $\leftarrow$ !ist} and 
% {\sf lvl' $\leftarrow$ indent} (lines~\ref{line:dref1},~\ref{line:dref2}). 
% Similarly, while reasoning about the {\it then} block,
% we need reasoning over the assignment expression {\sf ist := allowed} and {\sf ist := lvl'}.
% Thus, \name must be able to reason over such stateful expressions. \name\ 
% {\it natively} provides a static typing semantics for effectful expressions and computations discussed in Section ~\ref{sec:typing}. 
% \item Semantics of Parser Combinators, like the {\it Monadic-bind}, (hidden under the \M{do} statements), {\it Choice} (used in the definition of {\sf do\_}), and the {\it Kleene-star} (line~\ref{line:l2}).
% Unfortunately, extending our first-order specification language to type such higher-order and stateful combinators will either requires full power of expressive Higher-order logic~\cite{fstar,htt} which makes automatic type-checking undecidable or will require non-trivial bounds/relation annotations from the programmer~\cite{liquidextended,relref}.
% \end{itemize}


% An observation to make here is, that for most parser programs it suffices to use limited effects and a small set of 
% base combinators to build complex parsers. 
% \name uses this observation and axiomatizes (Section~\ref{sec:typing}) the semantics of the set of
% primitive parser combinators, thereby obviating the need for higher-order logic or infeasible user annotation burden.

% Given the types for these basic combinators 
% \name can synthesize a type for larger terms in a modular way.
% For example, using the type specifications for parser {\sf reserved} as follows-
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% @\begin{tabbing}  
% reserved : \{s : string $\mid$ true\} \=->\= $\mathsf{PE^{state}}$\= \{sel\= (h, ist) = I\}  
%               v : offsideTree I  \\
% \>\> \{\= sel (h, ist) = sel (h', ist) $\wedge$ indentT(v) = pos (sel (h, inp)\}
% \end{tabbing}@ 
% \end{lstlisting}  
% and {\sf indentedDoBlock} specification defined earlier, and
% the axiomatized semantics for monadic sequencing of parsers
% \name infers the following type:
% \vspace*{-.2in}
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% @\begin{tabbing}  
% \quad\quad\=$\mathsf{PE^{state}}$\= \{sel\= (h, ist) = I\} \\
% \>\>\>v : (offsideTree I) list\\
% \>\>      \{\=string (term (x)) = "do" $\wedge$ 
%           sel (h, ist) = sel (hi, ist) $\wedge$ sel (hi, ist) = sel (h', ist) $\wedge$ \\
% \>\>\>          indentT (dot) = pos (sel (h, inp))\}
% \end{tabbing}@      
% \end{lstlisting}
% for the following term (shown as a \M{do} statement (lines~\ref{line:do}-~\ref{line:ds})).  
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%   t = (reserved ''do'' @>>=\@ $\lambda$@ dot. indentedDoBlock)
% \end{lstlisting}

% Here {\sf dot} is a free variable occurring in the environment binding
% the result and \S{hi} is a free variable representing the
% intermediate result produced by applying the \S{reserved} parser to
% ``\S{do}''.  
% Intuitively, this inferred type says that
% the combined-parser's output is a list of (offsideTree I), and that if
% both parsers individually guarantee the \emph{reset} property, then by
% transitivity of equality, the combined parser guarantees this property
% as well. Further, if the first parser satisfies the {\it indentation}
% property then the combined parser also satisfies the property against
% the initial value of {\sf ist} in the input heap.

% Our axiomatization strategy would be clearly infeasible if we needed
% to axiomatize the semantics of each of these derived
% combinators. However, since their definitions are derived from a small
% fixed set of primitive combinators with simple axiomatizations and
% other type-checkable \name\ expressions, their types can be automatically
% inferred.

% For instance, given the earlier definition of {\sf star p}, and given a correct type for {\sf p} (i.e. \S{indentedDo} in
% our running example) and the required type for {$\mathsf{p_{star}}$} (i.e., the
% required type for \S{many \ indentedDo}), the type-checker uses the
% semantics of the fixpoint combinator to verify that 
% \S{many indentedDo} is well-typed by generating SMT-dischargable verification conditions and checking their validity.

% %\AM{The following can be removed as it does not give any new information other than details which can be burdensome at this point.}

% % As mentioned earlier, besides primitive parser combinators like
% % monadic sequencing, \name\ also provides a library of derived
% % combinators; for instance, the {\sf many} combinator (used at
% % line~\ref{line:l2}) is derived using the primitive fixpoint,
% % sequencing, and choice combinators:
% % \vspace*{-.2in}
% % \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% % @\begin{tabbing}
% % \quad\quad\ let many p = fix ($\lambda$\,\=p$_{\mathsf{star}}$ : $\tau$. \=map ($\lambda$\,\_ . []) eps \\
% % \>\>		<|>\\
% % \>\>              (p >>= $\lambda$\,x. p$_{\mathsf{star}}$ >>= $\lambda$ xs. return (x :: xs)) 
% % \end{tabbing}@
% % \end{lstlisting}
% % Our axiomatization strategy would be clearly infeasible if we needed
% % to axiomatize the semantics of each of these derived
% % combinators. However, since their definitions are derived from a small
% % fixed set of primitive combinators with simple axiomatizations and
% % other type-checkable \name\ expressions, their types can be automatically
% % inferred.

% % For instance, given a correct type for {\sf p} (i.e. \S{indentedDo} in
% % our running example) and the required type for {$\mathsf{p_{star}}$} (i.e., the
% % required type for \S{many indentedDo}), the type-checker uses the
% % semantics of the fixpoint combinator to verify that 
% % \S{many indentedDo} is well-typed by generating SMT-dischargable verification conditions and checking their validity.


% \paragraph{Type Annotations and Inference}
% % \AM{What : No need to annotate types with each parser
% %     Why : To reduce the annotation burden}
% Although the examples given above have explicit \name type annotations with each parser,
% \name can prove that a complex parser (like DoBlock) satisfies the given safety property 
% requiring only limited annotations (i.e. the required goal specification shown in \textcolor{blue}{blue} and annotation for the parsers written using the recursion combinator, e.g. many indentedDo).
% The other annotation shown in \textcolor{gray}{gray} are inferred by \name.
% To achieve this, \name uses a {\it strongest post-condition} predicate-transformer semantics with each expression.
% Although standard loop-invariant inference techniques~\cite{loop-invariant} can be applied for recursive functions, for our current implementation we assume a type provided by the programmer for recursive functions.

% % The typing rules in Sec~\ref{sec:typing} present rules for inferring logical effects each statement has on the algebraic data types as well as mutable heaps/states and compose these effects using the semantics for lambda expressions, combinators and let bindings to describe the effect for whole. 
% To illustrate, consider the {\sf indentedDo} parser, using the axiomatic semantics for the (\S{>>=}) and recursively inferring specifications
% for the {\sf do\_} parser (not shown for brevity, but in turn uses semantics for \S{>>=}, {\sf <|>}) and constructor definitions, 
% \name infers the following type for the {\sf indentedDo}.
% \vspace*{-.2in}
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%  @\begin{tabbing}  
% \quad\quad\=$\mathsf{PE^{state}}$\= \{sel\= (h, ist) = I\} v : (offsideTree I) result\\
% \>\>      \{\
%             v = Inl (x) => string (term (x)) = "do" $\wedge$ 
%                 sel (h', ist) = sel (h, ist) $\wedge$  indentT (dot) = pos (sel (h, inp)) \\
                 
% \>\> $\wedge$ v = Inr (Err)  => sel (h', ist) = sel (h, ist) \}
% \end{tabbing}@ 
% \end{lstlisting}

% The {\sf Inr Err} case is corresponding post-condition for the {\it then} branch (line~\ref{line:l3}) while the {\sf Inl x} case is for the {\it else} branch (line~\ref{line:l4}). 

% % indentedDo : $\mathsf{PE^{state}}$\,\= \{sel\= (h, ist) = I\}\\ 
% % \>\>              v : offsideTree I  \\
% % \>          \{indentT (v) = pos (sel (h, inp)\}
% % \end{tabbing}}}@ 




% % \paragraph{Automatic Reasoning over Mutable States}
% % % \AM{Why : Why is it interesting
% % %   1. Automated Reasoning over mutable states require richer logics
% % % What : Linear Types vs Axioms
% % % How  }
% % \name\ provides references mapping locations to values to define mutable states, a feature important for writing easy and efficient stateful/data-dependent parsers.
% % Unfortunately, {\it mutability} and {\it aliasing} together are challenging to reason automatically~\cite{ynot} and 
% % require either a richer logic like separation~\cite{separation} which are infeasible for automatic reasoning~\cite{iris,htt} or requires a complex sub-structural type systems~\cite{wadler-linear, rust}.
% % We take a different approach based on our observations about parser states. To enable automated reasoning in presence of mutable references \name defines a simplified
% % memory abstraction which is enforced using syntactic restrictions in the language. 
% % We prove a {\it uniqueness} theorem(Sec ~\ref{sec:typing}) which guarantees that each mutable value in our program is 
% % always reachable by a unique {\it reference path}, this gives us similar guarantees like those provided by  
% % a {\it substructural} Type system while greatly reducing the annotation and verification burden. 

% % This imposes aliasing restrictions on how objects
% % in the store may be shared; in particular, the language enforces the
% % constraint that there are a finite collection of references to mutable
% % shared state which are not subject to aliasing or implicit sharing
% % (i.e., guaranteed to be uniquely bound) when a reference is being updates. 
% % However like Linear Types~\cite{lineartype}, sharing is allowed for reading a 
% % reference. 
% % We have found that this
% % restriction imposes little burden on applications but allows us to
% % automate type-checking by avoiding the need to reason over complex
% % shared heap structures that are rarely found in parser applications.

% \subsection{Multiple effecs and Effect Local Typing}
% \label{subsec:efflocal}
% \AM{I feel this section could be removed as we can not do justice in explaination in this much space, and it might just confuse the reader.}
% %\AM{What Talk about the PE monad and fine grained effect}
% The Idris parser example shows that a parser may have multiple effects like states, exceptions and non-determinism. 
% A standard way of reasoning about such 
% programs is to either require the programmer to annotate a type capturing the semantics of each expression over the combined effect. Unfortunately this is infeasible for practical usages of \name and will break local reasoning. 
% To overcome this challenge, \name provides a fine-grained local reasoning over effect semantics of \name expression and parsers. Thus, each \name expression and computation is annotated
% with its local effect specification in a manner of effect-systems~\cite{param-monad-effect} and these local effect specifications are automatically 
% lifted into combined effect when these computations are composed. 

% For example, 
% consider the typing for the sequences \name expression ({\sf ist := allowed >>= fail "error" }).

% The inferred type for the statement {\sf ist := allowed} will be as follows:
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%   $\mathsf{PE^{state}}$ {true} v : unit  { update (h', h, ist, allowed)}  
% \end{lstlisting}
% The inferred type for the {\sf fail "error"} parser is as follows: 
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%   $\S{PE^{exc}}$ { $\forall$ $\S{h}$. $\S{true}$ } v  :  $\S{exc}$ {$\forall$ $\S{h}$, v, $\S{h'}$. h' = h $\wedge$ v = Err }  
% \end{lstlisting}

% % The parametric specification Monad {$\mathsf{PE^{\el}}$} is parameterized with the {\it effects} of the the computation it is specifying, 
% % the fine-grained type system in 
% \name then automatically lifts each of the above types into the type with {\it effects} for the composed statement.
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
%   $\S{PE^{st \sqcup exc}}$ {$\forall$ $\S{h}$. $\S{true}$ } v  :  $\S{exc}$ {$\forall$ $\S{h}$, v, $\S{h'}$. 
%   x = Err => h = h' $\wedge$ v = Err $\wedge$
%   x != Err => update ($\S{h'}$, $\S{h_i}$, ist, last)}  
% \end{lstlisting}
% where {\sf x} and $\S{h_i}$ are intermediate result and heap of evaluating the first expressions. (See Section~\ref{sec:typing} for details) 

\paragraph{Revisiting the Bug in the Example}
The bug described in Section~\ref{sec:ex} is unearthed while
typechecking the {\sf indentedDo} implementation.  To verify that
\S{doBlock} satisfies its specification, \name needs to prove
that the type inferred for the body of {\sf indentedDo}
(lines~\ref{line:idostart}-~\ref{line:l4}):

\begin{enumerate}
\item has a return type that is of the form, {\sf offsideTree I}.
  Concretely, the indentation of the returned tree must be greater
  than the initial value of {\sf ist} (i.e. indentT ($\nu$) > I).
  
\item asserts that the final value of {\sf ist} is equal to the
  initial value.
\end{enumerate}
Goal (1) is required because \textsf{indentedDo} is used by
\textsf{indentedDoBlock} (see Figure~\ref{fig:idris-original-do}),
which is then invoked by \textsf{doBlock}, where its result constructs
the value for \textsf{children}, whose type is \textsf{offsideTree I}
list.  Goal (2) is required because \S{doBlock}'s specified
post-condition demands it.

\noindent Typechecking the body for {\sf indentedDo} yields the following type:
  \vspace*{-.19in}
\begin{lstlisting}[escapechar=\@, basicstyle=\small\sf,language=ML]
@\texttt{\textcolor{black}{
  \begin{tabbing}                        
   $\mathsf{PE^{state}}$\,\= \{sel\= (h, ist) = I \}\\ 
  \>\>   $\nu$ : tree option  \\
  \>\{$\forall$ i : int.\=
   (i <= I $\Rightarrow$ h' = h) $\wedge$ \\
  \>\>(i > I $\Rightarrow$ indentT ($\nu$) = pos (sel (h, inp) $\wedge$ children ($\nu$) = nil\} 
  \end{tabbing}}}@
\end{lstlisting}
The two conjuncts in the post-condition correspond to the {\it then}
(failure case) and {\it else} (success case) branch in the parser's
body. The failure conjunct asserts that the heap remains unchanged if
the indentation level is greater than \textsf{ist}. The success
conjunct is the post-condition of the \textsf{do\_} parser. Clearly,
this inferred type, which specifies a return value of type \S{tree \
  option} is too weak to prove goal (1) given above, which requires
the combinator to return a parse tree that respects the offside rule.
The problem is that {\sf indent}'s type, inferred as {\sf indent :
  $\mathsf{PE^{state}}$ \{true\} $\nu$\, :\, int\, \{ h' = h \}}, does
not allow us to conclude that \S{indentedDo} satisfies the indentation
condition demanded by \S{doBlock}, i.e., that it returns a well-typed
(\S{offsideTree} I). This is because the type for {\sf indent} imposes
no constraint between the integer it returns and the function's input
heap, and thus offers no guarantees that its result gives the position
of the first lexeme of the input list.

% Given this specification, \name\ tries to prove a weaker implication (\S{i > sel (h, ist)} $\Rightarrow$
% \S{indentT(v)} > \S{sel (h, ist)}), which it fails as there is no relation between the 
% \S{indentT(v)} and \S{i}, and thus the program is flagged as
% ill-typed.
%% Unaware of this, the {\sf indentedDo} implementation assumes that the offside property is guaranteed by the {\sf indent}, the conditional
%% check at line~\ref{line:l3}, and the type for {\sf do\_} parser. To
%% illustrate, if a {\it revised} {\sf indent} function returns the correct position
%% {\sf i} of the next lexeme to be parsed, then the check at
%% line~\ref{line:l3} will ensure that the indentation of this lexeme is
%% greater than the current value of {\sf ist} and since {\sf indent}
%% does not consume the input, the position of the first lexeme for {\sf
%%   do\_} parser remains the same as {\sf i}. Thus, exploiting the
%% property of the {\sf do\_} that (\S{indentT(v) = pos (sel (h, inp)});
%% the constraint from the conditional check (\S{i} > \S{allowed}); the
%% obvious semantics of {\sf if-then-else}; the definition of {\sf offsideTree I}, we can prove the required
%% \S{offsideTree} property for \S{indentDo}'s return value  i.e. concretely \name will try to verify that
%% (\S{indentT(v) = pos (sel h, inp} $\wedge$ \S{i} = pos (sel h, inp)  $\wedge$ \S{i} > \S{sel (h, ist)} $\Rightarrow$
%%   \S{indentT(v)} > \S{sel (h, ist)}), which will hold and will not lead to the bug shown in the example. 

% \SJ{Perhaps give another implementation for indent and show that its specification is what is given below.}
% \AM{I felt, giving the revised spec for sourceColumn was more comprehensible than a revised implementation.}
If we revise the implementation of {\sf sourceColumn} such that it
always returns the position of the first element of the input list,
allowing us to track the indentation of every lexeme, the revised
inferred specifications for {\sf sourceColumn} and consequently for
{\sf indent} become:
\vspace*{-.2in}
\begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
@\texttt{\textcolor{black}{  
\begin{tabbing}
sourceColumn : (l : (char * int) list) -> \{$\nu$ : int | $\nu$ = pos (l)\} 
\end{tabbing}
}}@
@\texttt{\textcolor{black}{  
indent : $\mathsf{PE^{state}}$ \{true\} $\nu$ : int  \{$\nu$ = pos (sel (h, inp)) $\wedge$ h' = h\}}}@ 
\end{lstlisting}

Typechecking the {\sf indentedDo} implementation using this
strengthened specification for {\sf indent}
%\vspace*{-.2in}
% \begin{lstlisting}[escapechar=\@,basicstyle=\small\sf,language=ML]
% @\texttt{\textcolor{black}{  
% \quad\quad   indent : $\mathsf{PE^{state}}$ \{true\} $\nu$ : int  \{ $\nu$ = pos (sel (h, inp) $\wedge$ sel (h, ist) = sel (h', ist)\}}}@ 
% \end{lstlisting}
is succesful.  For this example, Morpheus generated {\sf 33}
Verification Conditions (VCs) for the revised successful case and {\sf
  6} VCs for the failing case. We were able to discharge these VCs to the SMT Solver
Z3~\cite{z3}, yielding a total overall verification time of {\sf
  10.46} seconds in the successful case, and {\sf 2.06} seconds in the
case when type-checking failed.


